Enhancement in tunneling density of states in Luttinger liquid -- role of non-local interaction

Power law suppression of local electronic tunneling density of states (TDOS) in the zero-energy limit is a hallmark of Luttinger liquid (LL) phase of the interacting 1-D electron system. We present a theoretical model which hosts LL state with the surprising feature of enhancement rather than suppression in local TDOS originating from non-local and repulsive density-density interactions. Importantly, we find enhancement of TDOS in the manifold of parameter space where the system is stable in the renormalization group (RG) sense. We argue that enhancement of TDOS along with RG stability is possible only when the system has broken parity symmetry about the position of local TDOS enhancement. Such a model could be realized on the edge states of a bi-layer quantum Hall system where both intra-layer and inter-layer density-density interactions are present mimicking the role of local and non-local interactions respectively.

==> TDOS1.tex <==
\bibitem{Kane1992}
C. L. Kane and M. P. A. Fisher, {\href{https://doi.org/10.1103/PhysRevB.46.15233}{Phys. Rev. B 46, 15233 (1992)}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{Yoreg1996}
Y. Oreg and A. M. Finkel'stein, {\href{https://doi.org/10.1103/PhysRevLett.76.4230}{Phys. Rev. Lett. 76, 4230 (1996)}}; M. Fabrizio and A. O. Gogolin, {\href{https://doi.org/10.1103/PhysRevLett.78.4527}{Phys. Rev. Lett. 78, 4527 (1997)}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bibitem{Fazio}
C. Winkelholz, R. Fazio, F. W. J. Hekking, and G. Schon, {\href{https://doi.org/10.1103/PhysRevLett.77.3200}{Phys. Rev. Lett. 77, 3200 (1996)}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{Fradkin}
E. Fradkin, {\href{https://arxiv.org/abs/cond-mat/9905218}{	arXiv:cond-mat/9905218}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{Eggert2000}
S. Eggert, {\href{https://doi.org/10.1103/PhysRevLett.84.4413}{Phys. Rev. Lett. 84, 4413 (2000)}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bibitem{kakashvili}
P. Kakashvili, H. Johannesson, and S. Eggert, {\href{https://doi.org/10.1103/PhysRevB.74.085114}{Phys. Rev. B 74, 085114 (2006)}}
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{Fisher-Glazman}
M. P. A. Fisher  and  L. I. Glazman, {\href{https://arxiv.org/pdf/cond-mat/9610037}{arXiv:cond-mat/9610037}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{Aristov2010}
D. N. Aristov, A. P. Dmitriev, I. V. Gornyi, V. Yu. Kachorovskii, D. G. Polyakov, and P. Wölfle, {\href{https://doi.org/10.1103/PhysRevLett.105.266404}{Phys. Rev. Lett. 105, 266404 (2010)}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bibitem{SDSarma2020}
D. Vu, A. Iucci, and S. Das Sarma, {\href{}{Phys. Rev. Res. 2, 023246 (2020)}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{Anderson}
P. W. Anderson, {\href{https://doi.org/10.1103/PhysRevLett.18.1049}{Phys. Rev. Lett. 18, 1049 (1967)}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{Ogawa}
T. Ogawa, A. Furusaki, and N. Nagaosa, {\href{https://doi.org/10.1103/PhysRevLett.68.3638}{Phys. Rev. Lett. 68, 3638 (1992)}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bibitem{Chen1992}
D. K. K. Lee and Y. Chen, {\href{https://doi.org/10.1103/PhysRevLett.69.1399}{Phys. Rev. Lett. 69, 1399 (1992)}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bibitem{gogolin1992}
A. O. Gogolin, {\href{https://doi.org/10.1103/PhysRevLett.71.2995}{Phys. Rev. Lett. 71, 2995 (1993)}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bibitem{prokofev}
N. V. Prokof'ev, {\href{https://doi.org/10.1103/PhysRevB.49.2148}{Phys. Rev. B 49, 2148 (1994)}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bibitem{Glazman_kane}
C. L. Kane, K. A. Matveev, and L. I. Glazman, {\href{https://doi.org/10.1103/PhysRevB.49.2253}{Phys. Rev. B 49, 2253 (1994)}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bibitem{Affleck_ludwig}
I. Affleck and A. W. W. Ludwig, {\href{https://iopscience.iop.org/article/10.1088/0305-4470/30/16/017/meta}{J. Phys. A: Math. Gen. 27, 5375 (1994).}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bibitem{Finkelstein1996}
Y. Oreg and A. M. Finkelstein, {\href{https://doi.org/10.1103/PhysRevB.53.10928}{Phys. Rev. B 53, 10928 (1996)}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bibitem{Furusaki}
A. Furusaki, {\href{https://doi.org/10.1103/PhysRevB.56.9352}{Phys. Rev. B 56, 9352 (1997)}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{Haldane}
F D M Haldane, {\href{https://iopscience.iop.org/article/10.1088/0022-3719/14/19/010/meta}{ J. Phys. C: Solid State Phys. 14 2585 (1981)}}
\bibitem{Meden_voit}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

K. Schönhammer and V. Meden, {\href{https://doi.org/10.1103/PhysRevB.47.16205}{Phys. Rev. B 47, 16205 (1993)}}; J. Voit, {\href{https://iopscience.iop.org/article/10.1088/0953-8984/5/44/020}{J. Phys.: Cond. Mat. 5, 8305 (1993)}} 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{JVDelft}
Jan von Delft and Herbert Schoeller, {\href{https://doi.org/10.1002/(SICI)1521-3889(199811)7:4<225::AID-ANDP225>3.0.CO;2-L}{Ann. Phys. (Berlin) 7, 225 (1998).}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{gogolinbook}
A. O. Gogolin, A. A. Nersesyan, A. M. Tsvelik, {\href{https://arxiv.org/abs/cond-mat/9909069}{	arXiv:cond-mat/9909069}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{SRao}
Sumathi Rao and Diptiman Sen, {\href{https://arxiv.org/abs/cond-mat/0005492}{ in {\it{Field Theories in Condensed Matter Physics}} (Kluwer, Dordrecht, 2001), pp. 239–333.}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{Giamarchi}
T. Giamarchi, {\it{Quantum Physics in One Dimension}} (Oxford University Press, Oxford, 2004)

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{Maslov}
Dmitrii L. Maslov, {\href{https://arxiv.org/abs/cond-mat/0506035}{	arXiv:cond-mat/0506035}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5

\bibitem{Nancy}
N. P. Sandler, C. Chamon, and E. Fradkin, {\href{https://doi.org/10.1103/PhysRevB.57.12324}{Phys. Rev. B 57, 12324 (1998)}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{Chklovskii1998}
Dmitri B. Chklovskii and Bertrand I. Halperin, {\href{https://journals.aps.org/prb/abstract/10.1103/PhysRevB.57.3781}{Phys. Rev. B 57, 3781(1998)}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bibitem{Sen2008}
Diptiman Sen and Amit Agarwal, {\href{https://journals.aps.org/prb/abstract/10.1103/PhysRevB.78.085430}{Phys. Rev. B 78, 085430(2008)}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bibitem{Wen}
X. G. Wen, {\href{https://doi.org/10.1103/PhysRevB.41.12838}{Phys.Rev.B 41, 12838-12844 (1990)}}; X. -G. Wen,{\href{https://doi.org/10.1103/PhysRevLett.64.2206}{Phys. Rev. Lett. 64, 2206 (1990)}}; X. G. Wen,{\href{https://doi.org/10.1103/PhysRevB.44.5708}{Phys. Rev. B 44, 5708 (1991)}};  X. -G. Wen,{\href{https://doi.org/10.1103/PhysRevB.43.11025}{Phys. Rev. B 43, 11025 (1991)}}; X. -G. Wen, {\href{https://doi.org/10.1142/S0217979292000840}{Int.J.Mod.Phys. B6 (1992) 1711-1762}}; X. -G. Wen, {\href{https://journals.aps.org/prb/abstract/10.1103/PhysRevB.50.5420}{Phys. Rev. B 50, 5420 (1994)}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{Nayak1999}
C. Nayak, M. P. A. Fisher, A. W. W. Ludwig, and H. H. Lin, {\href{https://doi.org/10.1103/PhysRevB.59.15694}{Phys. Rev. B 59, 15694 (1999)}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{Meden2000}
V. Meden, W. Metzner, U. Schollwöck, O. Schneider, T. Stauber,
and K. Schönhammer, {\href{https://link.springer.com/article/10.1007/s100510070180}{Eur. Phys. J. B 16(4) 631646 (2000)}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{SLal2002}
S. Lal, S. Rao, and D. Sen, {\href{https://doi.org/10.1103/PhysRevB.66.165327}{Phys. Rev. B 66, 165327 (2002)}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{chang2003}
A. M. Chang, {\href{https://doi.org/10.1103/RevModPhys.75.1449}{Rev. Mod. Phys. 75, 1449 (2003)}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{Egger2003}
R. Egger, B. Trauzettel, S. Chen, and F. Siano, {\href{https://iopscience.iop.org/article/10.1088/1367-2630/5/1/117}{ New J. Phys. 5, 117 (2003)}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{chamon2003}
C. Chamon, M. Oshikawa, and I. Affleck, {\href{https://doi.org/10.1103/PhysRevLett.91.206403}{Phys. Rev. Lett. 91, 206403 (2003)}}, M. Oshikawa, C. Chamon, and I. Affleck, {\href{https://iopscience.iop.org/article/10.1088/1742-5468/2006/02/P02008}{ J. Stat. Mech.: Theory Exp. P02008 (2006)}}; A. Rahmani, Chang-Yu Hou, A. Feiguin, M. Oshikawa, C. Chamon, and I. Affleck, {\href{https://doi.org/10.1103/PhysRevB.85.045120}{Phys. Rev. B 85, 045120 (2012)}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{SDas2004}
S. Das, S. Rao, and D. Sen, {\href{https://doi.org/10.1103/PhysRevB.70.085318}{Phys. Rev. B 70, 085318 (2004)}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bibitem{Sedeki}
X. Barnabé-Thériault, A. Sedeki, V. Meden, and K. Schönhammer, {\href{https://doi.org/10.1103/PhysRevB.71.205327}{Phys. Rev. B 71, 205327 (2005)}}; X. Barnabé-Thériault, A. Sedeki, V. Meden, and K. Schönhammer, {\href{https://doi.org/10.1103/PhysRevLett.94.136405}{Phys. Rev. Lett. 94, 136405 (2005)}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bibitem{Guo2006}
H. Guo and S. R. White, {\href{https://doi.org/10.1103/PhysRevB.74.060401}{Phys. Rev. B 74, 060401(R) (2006)}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{SDas2006}
S. Das, S. Rao, and D. Sen, {\href{https://doi.org/10.1103/PhysRevB.74.045322}{Phys. Rev. B 74, 045322 (2006)}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{SDas2008}
S. Das, S. Rao, and A. Saha, {\href{https://doi.org/10.1103/PhysRevB.77.155418}{Phys. Rev. B 77, 155418 (2008)}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bibitem{Das2008}
S. Das and S. Rao, {\href{https://journals.aps.org/prb/abstract/10.1103/PhysRevB.78.205421}{ Phys. Rev. B 78, 205421(2008)}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{Chamon2008}
C.-Y. Hou and C. Chamon, {\href{https://doi.org/10.1103/PhysRevB.77.155422}{Phys. Rev. B 77, 155422 (2008)}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{Demler2008}
A. Tokuno, M. Oshikawa and E. Demler, {\href{https://doi.org/10.1103/PhysRevLett.100.140402}{ Phys. Rev. Lett. 100, 140402 (2008)}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{Schonhammer2009}
P. Wächter, V. Meden, and K. Schönhammer, {\href{https://iopscience.iop.org/article/10.1088/0953-8984/21/21/215608/meta}{J. Phys.: Condens. Matter 21, 215608 (2009)}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{SDas2009}
A. Agarwal, S. Das, S. Rao, and D. Sen, {\href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.103.026401}{Phys. Rev. Lett. 103, 026401 (2009)}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bibitem{Bellazzini2009}
B. Bellazzini, P. Calabrese, and M. Mintchev, {\href{https://doi.org/10.1103/PhysRevB.79.085122}{ Phys. Rev. B 79, 085122 (2009)}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{SDas2010}
A. Agarwal, S. Das, and D. Sen, {\href{https://doi.org/10.1103/PhysRevB.81.035324}{Phys. Rev. B 81, 035324 (2010)}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{Aristov2011}
D. N. Aristov and P. Wölfle, {\href{https://doi.org/10.1103/PhysRevB.84.155426}{Phys. Rev. B 84, 155426 (2011)}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{Rahmani}
A. Rahmani, C.-Y. Hou, A. Feiguin, C. Chamon, and I. Affleck, {\href{https://doi.org/10.1103/PhysRevLett.105.226803}{Phys. Rev. Lett. 105, 226803 (2010)}}; A. Rahmani, C.-Y. Hou, A. Feiguin, M. Oshikawa, C. Chamon, and I. Affleck, {\href{https://doi.org/10.1103/PhysRevB.85.045120}{Phys. Rev. B 85, 045120 (2012)}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{Altland_gefen}
A. Altland, Y. Gefen, and B. Rosenow, {\href{https://doi.org/10.1103/PhysRevLett.108.136401}{Phys. Rev. Lett. 108, 136401 (2012)}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{Aristov2013}
D. N. Aristov and P. Wölfle, {\href{https://doi.org/10.1103/PhysRevB.86.035137}{Phys. Rev. B 86, 035137 (2012)}}; D. N. Aristov and P. Wölfle, {\href{https://doi.org/10.1103/PhysRevB.88.075131}{Phys. Rev. B 88, 075131 (2013)}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{Agarwal2015}
S. Mardanya and A. Agarwal, {\href{https://doi.org/10.1103/PhysRevB.92.045432}{Phys. Rev. B 92, 045432 (2015)}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{shi2016}
Z. Shi and I. Affleck, {\href{https://doi.org/10.1103/PhysRevB.94.035106}{Phys. Rev. B 94, 035106 (2016)}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bibitem{Manu2016}
M. Kumar, A. Parvej, S. Thomas, S. Ramasesha, and Z. G. Soos,
{\href{https://doi.org/10.1103/PhysRevB.93.075107}{Phys. Rev. B 93, 075107 (2016)}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bibitem{Ramos2019}
F. Buccheri, R. Egger, R. G. Pereira and F. B. Ramos, {\href{https://doi.org/10.1016/j.nuclphysb.2019.03.005}{Nucl. Phys. B 941 794837 (2019)}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{Manu2020}
M. S. Roy, M. Kumar, and S. Das, {\href{https://doi.org/10.1103/PhysRevB.102.035130}{Phys. Rev. B 102, 035130 (2020)}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%55

\bibitem{kane_fisher}
C. L. Kane and M. P. A. Fisher, {\href{https://doi.org/10.1103/PhysRevLett.68.1220}{Phys. Rev. Lett. 68, 1220 (1992)}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{West1990}
G. S. Boebinger, H. W. Jiang, L. N. Pfeiffer, and K. W. West, {\href{https://doi.org/10.1103/PhysRevLett.64.1793}{Phys. Rev. Lett. 64, 1793 (1990)}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{Shayegan}
 Y. W. Suen, J. Jo, M. B. Santos, L. W. Engel, S. W. Hwang, and M. Shayegan, {\href{https://doi.org/10.1103/PhysRevB.44.5947}{Phys. Rev. B 44, 5947(R) (1991)}}; H. C. Manoharan, Y. W. Suen, T. S. Lay, M. B. Santos, and M. Shayegan, {\href{https://doi.org/10.1103/PhysRevLett.79.2722}{Phys. Rev. Lett. 79, 2722 (1997)}}; T. S. Lay, T. Jungwirth, L. Smrčka, and M. Shayegan, {\href{https://doi.org/10.1103/PhysRevB.56.R7092}{Phys. Rev. B 56, R7092(R) (1997)}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{Eisentein1992}
J. P. Eisenstein, G. S. Boebinger, L. N. Pfeiffer, K. W. West, and Song He, {\href{https://doi.org/10.1103/PhysRevLett.68.1383}{Phys. Rev. Lett. 68, 1383 (1992)}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bibitem{Eisentein}
J.P. Eisenstein, {\href{https://doi.org/10.1146/annurev-conmatphys-031113-133832}{Annual Review of Condensed Matter Physics, Vol. 5:159-181 (2014)}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{shankar1995}
R. Shankar, {\href{https://www.worldscientific.com/doi/abs/10.1142/9789814447027_0006}{Bosonization, in {\it{Low-Dimensional Quantum Field Theories for Condensed Matter Physicists}} (World Scientific, Singapore, 1995), pp. 353–387 }}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{DSen2009}
S. Das, S. Rao and D. Sen, {\href{https://iopscience.iop.org/article/10.1209/0295-5075/86/37010}{ EPL (Europhys. Lett.), 86, 37010 (2009)}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{Fisher1997}
M. P. A. Fisher, L. I. Glazman, Transport in a one-dimensional Luttinger liquid, in {\it{Mesoscopic Electron Transport}}, NATO ASI Series Vol. 345 (Springer, Dordrecht, 1997), pp. 331–373.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{laughlin1981}
R. B. Laughlin, {\href{https://doi.org/10.1103/PhysRevB.23.5632}{Phys. Rev. B 23, 5632(R) (1981)}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bibitem{Halperin1982}
B. I. Halperin, {\href{https://doi.org/10.1103/PhysRevB.25.2185}{Phys. Rev. B 25, 2185 (1982)}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{stormer1999}
H. L. Stormer, {\href{https://doi.org/10.1103/RevModPhys.71.875}{Rev. Mod. Phys. 71, 875 (1999)}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{Latief}
A. Latief and B. Beri, {\href{https://doi.org/10.1103/PhysRevB.98.205427}{Phys. Rev. B 98, 205427 (2018)}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{Barkeshi}
M. Barkeshli and X.-L. Qi, {\href{https://doi.org/10.1103/PhysRevX.4.041035}{Phys. Rev. X 4, 041035 (2014)}}; M. Barkeshli, {\href{https://doi.org/10.1103/PhysRevLett.117.096803}{Phys. Rev. Lett. 117, 096803 (2016)}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{Sarma2015}
M. R. Peterson, Y.-Le Wu, M. Cheng, M. Barkeshli, Z. Wang, and S. D. Sarma, {\href{https://doi.org/10.1103/PhysRevB.92.035103}{Phys. Rev. B 92, 035103 (2015)}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{Alicea2016}
J. Alicea and P. Fendley, {\href{https://doi.org/10.1146/annurev-conmatphys-031115-011336}{Annual Review of Condensed Matter Physics, Vol. 7:119-139 (2016)}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{Ebisu2017}
H. Ebisu, E. Sagi, Y. Tanaka, and Y. Oreg, {\href{https://doi.org/10.1103/PhysRevB.95.075111}{Phys. Rev. B 95, 075111 (2017)}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{Ensslin}
H. Overweg H. Eggimann, X. Chen, S. Slizovskiy, M. Eich, R. Pisoni, Y. Lee, P. Rickhaus, K. Watanabe, T. Taniguchi, V. Falko, T. Ihn, and K. Ensslin, {\href{https://pubs.acs.org/doi/10.1021/acs.nanolett.7b04666}{Nano Letters 2018 18 (1), 553-559}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\bibitem{Jun_Zhu}
J. Li, H. Wen, K. Watanabe, T. Taniguchi, and J. Zhu, {\href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.120.057701}{Phys. Rev. Lett. 120, 057701 }}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{Geim}
K. S. Novoselov, E. McCann, S. V. Morozov, V. I. Fal’ko, M. I. Katsnelson, U. Zeitler, D. Jiang, F. Schedin and A. K. Geim, {\href{https://www.nature.com/articles/nphys245}{Nature Physics volume 2, pages177–180(2006)}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%55
\bibitem{Abanin}
D.-K. Ki, V. I. Fal’ko, D. A. Abanin, and A. F. Morpurgo, {\href{https://pubs.acs.org/doi/10.1021/nl5003922}{Nano Lett. 2014, 14, 4, 2135–2139}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bibitem{Kou}
A. Kou, B. E. Feldman, A. J. Levin, B. I. Halperin, K. Watanabe, T. Taniguchi, A. Yacoby, {\href{https://science.sciencemag.org/content/345/6192/55.abstract}{Science 04 Jul 2014: Vol. 345, Issue 6192, pp. 55-57}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bibitem{Maher}
P. Maher, L. Wang, Y. Gao, C. Forsythe, T. Taniguchi, K. Watanabe, D. Abanin, Z. Papi´c, P. Cadden-Zimansky, J. Hone, P. Kim, and C. R. Dean,  {\href{https://science.sciencemag.org/content/345/6192/61.full}{Science  04 Jul 2014: Vol. 345, Issue 6192, pp. 61-64}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5

\bibitem{Kim}
Y. Kim, D. S. Lee, S. Jung, V. Sk´akalov´a, T. Taniguchi, K. Watanabe, J. S. Kim, and J. H. Smet, {\href{https://pubs.acs.org/doi/abs/10.1021/acs.nanolett.5b02876}{Nano Lett. 2015, 15, 11, 7445–7451}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\bibitem{Diankov}
G. Diankov, C.-T. Liang, F. Amet, P. Gallagher, M. Lee, A. J. Bestwick, K. Tharratt, W. Coniglio, J. Jaroszynski, K. Watanabe, T. Taniguchi, and D. Goldhaber-Gordon, {\href{https://www.nature.com/articles/ncomms13908}{Nat. Commun. 7, 13908 (2016)}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{Hashisaka}
H. Kamata, N. Kumada, M. Hashisaka, K. Muraki, and T. Fujisawa {\href{https://doi.org/10.1038/nnano.2013.312}{ Nat. Nanotechnol. 9, 177–181 (2014)}}; M. Hashisaka, H. Kamata, N.
Kumada, K. Washio, R. Murata, K. Muraki, and T. Fujisawa, {\href{https://journals.aps.org/prb/abstract/10.1103/PhysRevB.88.235409}{Phys. Rev. B 88, 235409 (2013)}}, 
M. Hashisaka and T. Fujisawa, {\href{https://doi.org/10.1016/j.revip.2018.07.001}{Rev. Phys. 3, 32 (2018)}}





